AI exposure predicts unemployment risk

Is artificial intelligence (AI) disrupting jobs and creating unemployment? Despite many attempts to quantify occupations' exposure to AI, inconsistent validation obfuscates the relative benefits of each approach. A lack of disaggregated labor outcome data, including unemployment data, further exacerbates the issue. Here, we assess which models of AI exposure predict job separations and unemployment risk using new occupation-level unemployment data by occupation from each US state's unemployment insurance office spanning 2010 through 2020. Although these AI exposure scores have been used by governments and industry, we find that individual AI exposure models are not predictive of unemployment rates, unemployment risk, or job separation rates. However, an ensemble of those models exhibits substantial predictive power suggesting that competing models may capture different aspects of AI exposure that collectively account for AI's variable impact across occupations, regions, and time. Our results also call for dynamic, context-aware, and validated methods for assessing AI exposure. Interactive visualizations for this study are available at https://sites.pitt.edu/~mrfrank/uiRiskDemo/.

==> tables/uiOLS.tex <==
\tiny
\begin{tabularx}{\textwidth}{l|XXXXXXXXXXX}
\hline
\multicolumn{12}{c}{Dependent Variable: Log$_{10}$ Unemployment Risk by Occupation, Month, \& State} \\ \hline
                                                                       Variable &                         Model 1 &                         Model 2 &                        Model 3 &                        Model 4 &                        Model 5 &                        Model 6 &                         Model 7 &                         Model 8 &                         Model 9 &          Model 10 &                        Model 11 \\
          Acemoglu \& Autor$^{[14]}$&         \multirow{2}{*}{-0.000} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} &  \multirow{2}{*}{0.527$^{***}$} & \multirow{2}{*}{} &  \multirow{2}{*}{0.562$^{***}$} \\
 Computer Usage &&&&&&&&&&& \\
       Acemoglu \& Autor$^{[14]}$& \multirow{2}{*}{-0.074$^{***}$} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.155$^{***}$} & \multirow{2}{*}{} & \multirow{2}{*}{-0.184$^{***}$} \\
 Routine Cognitive &&&&&&&&&&& \\
          Acemoglu \& Autor$^{[14]}$ &  \multirow{2}{*}{0.109$^{***}$} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.131$^{***}$} & \multirow{2}{*}{} & \multirow{2}{*}{-0.084$^{***}$} \\
 Routine Manual &&&&&&&&&&& \\
                        ONET &               \multirow{2}{*}{} & \multirow{2}{*}{-0.111$^{***}$} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} &         \multirow{2}{*}{-0.000} & \multirow{2}{*}{} &          \multirow{2}{*}{0.000} \\
 \% Bachelors &&&&&&&&&&& \\ 
  Frey \& Osborne$^{[17]}$ &               \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{0.014$^{***}$} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.066$^{***}$} & \multirow{2}{*}{} & \multirow{2}{*}{-0.027$^{***}$} \\
 Prob. of Computerisation &&&&&&&&&&& \\
                  Arntz et al$^{[18]}$&               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} & \multirow{2}{*}{0.273$^{***}$} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} &  \multirow{2}{*}{0.599$^{***}$} & \multirow{2}{*}{} &  \multirow{2}{*}{0.565$^{***}$} \\
 Probability &&&&&&&&&&& \\
              ONET Degree &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} & \multirow{2}{*}{0.129$^{***}$} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &               \multirow{2}{*}{} &  \multirow{2}{*}{0.028$^{***}$} & \multirow{2}{*}{} &          \multirow{2}{*}{0.000} \\
of Automation &&&&&&&&&&& \\
    Brynjolfsson et al$^{[23]}$ &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} & \multirow{2}{*}{0.072$^{***}$} &               \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.155$^{***}$} & \multirow{2}{*}{} & \multirow{2}{*}{-0.145$^{***}$} \\
 Suitability for ML &&&&&&&&&&& \\
                 Felten et al$^{[24]}$  &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} & \multirow{2}{*}{-0.095$^{***}$} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.117$^{***}$} & \multirow{2}{*}{} & \multirow{2}{*}{-0.114$^{***}$} \\
AI Exposure &&&&&&&&&&& \\
                                Webb$^{[25]}$ \% AI &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &  \multirow{2}{*}{0.278$^{***}$} &         \multirow{2}{*}{-0.000} & \multirow{2}{*}{} &         \multirow{2}{*}{-0.000} \\
&&&&&&&&&&& \\
                             Webb$^{[25]}$ \% Robot &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} &  \multirow{2}{*}{0.337$^{***}$} &  \multirow{2}{*}{0.372$^{***}$} & \multirow{2}{*}{} &  \multirow{2}{*}{0.358$^{***}$} \\
&&&&&&&&&&& \\
                          Webb$^{[25]}$ \% Software &               \multirow{2}{*}{} &               \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &              \multirow{2}{*}{} &               \multirow{2}{*}{} & \multirow{2}{*}{-0.237$^{***}$} &         \multirow{2}{*}{-0.000} & \multirow{2}{*}{} &         \multirow{2}{*}{-0.000} \\
&&&&&&&&&&& \\
                                         \hline Year F.E. &                              No &                              No &                             No &                             No &                             No &                             No &                              No &                              No &                              No &               Yes &                             Yes \\
                                        Month F.E. &                              No &                              No &                             No &                             No &                             No &                             No &                              No &                              No &                              No &               Yes &                             Yes \\
                                        State F.E. &                              No &                              No &                             No &                             No &                             No &                             No &                              No &                              No &                              No &               Yes &                             Yes \\
                                             \hline
$R^2$ &                           0.017 &                           0.012 &                          0.000 &                          0.075 &                          0.017 &                          0.005 &                           0.009 &                           0.063 &                           0.204 &             0.605 &                           0.788 \\
                                        adj. $R^2$ &                           0.017 &                           0.012 &                          0.000 &                          0.075 &                          0.017 &                          0.005 &                           0.009 &                           0.063 &                           0.204 &             0.604 &                           0.787 \\
\hline \multicolumn{12}{c}{$p_{val}<0.1^*$, $p_{val}<0.01^{**}$, $p_{val}<0.001^{***}$} \\ \hline
\end{tabularx}
